AF-Muon: An AdamW-Free Muon Optimizer for Tied-Embedding Models

Muon improves large-scale training by applying a spectral-norm steepest-descent update to matrix parameters, but practical models also contain parameter blocks that do not fit dense-matrix geometry. One important case is the tied vocabulary table, which appears in language models and other token generators and can receive multiple structurally different gradient sources, from sparse input lookups to dense output-classifier updates. In the reference recipe these blocks are handed to an auxiliary AdamW optimizer, which restores second-moment state and updates the aliased table as a generic tensor. We propose AF-Muon, an AdamW-free extension of Muon that keeps the Muon matrix update for hidden weight matrices while using a support-aware finite-cap linear minimization oracle for tied vocabulary tables and an RMS-normalized update for one-dimensional auxiliary parameters. AF-Muon therefore trains every parameter class with a single first-moment buffer and no second-moment state, saving around 20% optimizer-state memory relative to Hybrid Muon in our benchmark. Across nine tied-token settings - decoder-only language models from 124M to 1B parameters, a fully shared T5-style encoder-decoder, and ImageGPT-style image-token, protein, and sparse-MoE variants, spanning text, image, and protein-sequence data - AF-Muon improves mean validation loss and perplexity over both Hybrid Muon and a SCION-style Sign endpoint. Long-horizon runs and hyperparameter sensitivity studies confirm the gain is robust, and identical-momentum diagnostics attribute it to the finite cap, which preserves more within-row magnitude than Sign while bounding the coordinate concentration of row-RMS. These results identify tied vocabulary tables as a distinct optimizer geometry and yield a robust AdamW-free Muon variant across models, modalities, and architectures, with about 1% step-time overhead in matched training.

==> figs/Intersection-norm.tex <==
\begin{tikzpicture}
  % \begin{axis}[
  %   xlabel={$X_1$},
  %   ylabel={$X_2$},
  %   xmin=-2.5, xmax=2.5,
  %   ymin=-2.0, ymax=2.0,
  %   xtick={-2, -1, 0, 1, 2},
  %   ytick={-2.0, -1.5, -1.0, -0.5, 0.0, 0.5, 1.0, 1.5, 2.0},
  %   yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=1},
  %   grid=major,
  %   grid style={dotted, gray!40},
  %   axis line style={gray!80},
  %   tick label style={font=\small},
  %   label style={font=\medium},
  %   width=8cm, height=6.5cm,
  %   legend pos=north east,
  %   legend style={font=\footnotesize, fill=white, fill opacity=0.9, draw opacity=0.7}
  % ]
\begin{axis}[
    title style={font=\large, yshift=3pt},
    xlabel={$X_1$},
    ylabel={$X_2$},
    xmin=-2.5, xmax=2.5,
    ymin=-2.0, ymax=2.0,
    xtick={-2, -1, 0, 1, 2},
    ytick={-2.0, -1.5, -1.0, -0.5, 0.0, 0.5, 1.0, 1.5, 2.0},
    yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=1},
    grid=major,
    grid style={dotted, gray!40},
    axis line style={gray!80},
    tick label style={font=\small},
    label style={font=\small},
    width=10cm, height=8cm,
    legend pos=north east,
    legend style={
      font=\footnotesize, 
      fill=white, 
      fill opacity=0.9, 
      draw opacity=0.7
    },
    every legend image post/.append style={scale=0.6}
  ]

    % Main coordinate axes lines (x=0, y=0)
    \draw[gray!70, line width=0.6pt] (axis cs:-2.5, 0) -- (axis cs:2.5, 0);
    \draw[gray!70, line width=0.6pt] (axis cs:0, -2) -- (axis cs:0, 2);

    % Constraint Set 1 (Light Blue Circle)
    \fill[set1color, opacity=0.75] (axis cs:-0.5, 0) circle [radius=1.5];

    % Constraint Set 2 (Light Green Circle)
    \fill[set2color, opacity=0.65] (axis cs:0.5, 0) circle [radius=1.2];

    % Shared Feasible Region (Clipped Vertical Strip)
    \begin{scope}
      \clip (axis cs:-0.2, -2) rectangle (axis cs:0.2, 2);
      \fill[sharedcolor, opacity=0.9] (axis cs:-0.5, 0) circle [radius=1.5];
    \end{scope}

    % Start Point
    \fill[black] (axis cs:-1.5, 1.2) circle (2.5pt) 
      node[above=3pt, font=\small, color=black] {Start};

    % Update Vector U (Arrow)
    \draw[->, >=stealth, color=vectorcolor, line width=3.5pt, shorten >=3pt] 
      (axis cs:-1.5, 1.2) -- (axis cs:0, 0.1);

    % Vector Label U
    \node[color=vectorcolor, font=\large\bfseries\itshape] at (axis cs:0.0, 0.35) {$U$};

    % Endpoint Marker
    \fill[vectorcolor] (axis cs:0, 0.1) circle (3pt);

    % Legend Setup
    \addlegendimage{only marks, mark=square*, mark size=2.5pt, color=set1color, opacity=0.75} % reduced from 4pt
    \addlegendentry{Constraint Set 1}
    
    \addlegendimage{only marks, mark=square*, mark size=2.5pt, color=set2color, opacity=0.65} % reduced from 4pt
    \addlegendentry{Constraint Set 2}
    
    \addlegendimage{only marks, mark=square*, mark size=2.5pt, color=sharedcolor, opacity=0.9} % reduced from 4pt
    \addlegendentry{Shared Feasible Region}
    
    \addlegendimage{line width=2pt, color=vectorcolor} % reduced from 4pt
    \addlegendentry{Update Vector $U$}

  \end{axis}
\end{tikzpicture}

==> figs/shared-region.tex <==
\begin{tikzpicture}[scale=0.95, >=Stealth]

  % --- Top Header Text ---
  % \node[align=center, font=\sffamily] at (2.2, 3.8) {
  %   \large\textcolor{afmgray}{increasing $c \longrightarrow$ weaker coordinate cap} \\[3pt]
  %   \small\textcolor{afmgray}{same oracle input $b$; illustrative $d_{\text{vis}} = 16$}
  % };

  % =========================================================
  % PANEL 1: c = 1 (Sign)
  % =========================================================
  \begin{scope}[shift={(-3.2,0)}]
    % Title
    \node[align=center, font=\sffamily\small] at (0, 2.1) {
      \textcolor{afmgray}{$c=1$} \\
      \textcolor{afmgray}{Sign}
    };
    
    % Coordinate axes
    \draw[afmlinegray, thin] (-1.5,0) -- (1.5,0);
    \draw[afmlinegray, thin] (0,-1.5) -- (0,1.5);
    
    % Outer row-l2 circle
    \draw[afmgray, thick] (0,0) circle (1.2);
    
    % Small dashed max-entry box (c=1)
    \draw[afmgray, thick, dashed] (-0.3, -0.3) rectangle (0.3, 0.3);
    
    % Oracle direction dot
    \fill[afmgray] (0.45, 0.2) circle (1.5pt);
    
    % Update vector
    \draw[->, afmgray, thick] (0,0) -- (-0.18, -0.15);
    
    % Subscript label
    \node[font=\sffamily] at (0, -1.8) {\textcolor{afmgray}{$u_1^*$}};
  \end{scope}

  % =========================================================
  % PANEL 2: c = 3 (AF-Muon)
  % =========================================================
  \begin{scope}[shift={(0.4,0)}]
    % Title
    \node[align=center, font=\sffamily\small] at (0, 2.1) {
      \textcolor{afmmagenta}{\textbf{$c=3$}} \\
      \textcolor{afmmagenta}{\textbf{AF-Muon}}
    };
    
    % Coordinate axes
    \draw[afmlinegray, thin] (-1.5,0) -- (1.5,0);
    \draw[afmlinegray, thin] (0,-1.5) -- (0,1.5);
    
    % Shared intersection fill
    \begin{scope}
      \clip (0,0) circle (1.2);
      \fill[afmgreen!70!white] (-0.85, -0.85) rectangle (0.85, 0.85);
    \end{scope}
    
    % Max-entry ball (orange box)
    \draw[afmorange, ultra thick] (-0.85, -0.85) rectangle (0.85, 0.85);
    
    % Row-l2 ball (blue circle)
    \draw[afmblue, ultra thick] (0,0) circle (1.2);
    
    % Origin point
    \fill[black] (0,0) circle (1.5pt);
    
    % Update vector arrow
    \draw[->, afmmagenta, line width=2.5pt] (0,0) -- (0.78, 0.78);
    
    % Endpoint marker
    \fill[afmmagenta] (0.85, 0.85) circle (3pt);
    \fill[white] (0.85, 0.85) circle (1.2pt);
    
    % Subscript label
    \node[font=\sffamily] at (0, -1.8) {\textcolor{afmmagenta}{$u_3^*$}};
  \end{scope}

  % =========================================================
  % PANEL 3: c = 5 (Relaxed Cap)
  % =========================================================
  \begin{scope}[shift={(4.0,0)}]
    % Title
    \node[align=center, font=\sffamily\small] at (0, 2.1) {
      \textcolor{afmgray}{$c=5$} \\
      \textcolor{afmgray}{relaxed cap}
    };
    
    % Large dashed max-entry box (c=5)
    \draw[afmgray, thick, dashed] (-1.4, -1.4) rectangle (1.4, 1.4);
    
    % Coordinate axes
    \draw[afmlinegray, thin] (-1.5,0) -- (1.5,0);
    \draw[afmlinegray, thin] (0,-1.5) -- (0,1.5);
    
    % Inner row-l2 circle
    \draw[afmgray, thick] (0,0) circle (1.2);
    
    % Origin point
    \fill[black] (0,0) circle (1.5pt);
    
    % Update vector arrow
    \draw[->, afmgray, ultra thick] (0,0) -- (1.02, 0.63);
    
    % Endpoint marker
    \fill[afmgray] (1.02, 0.63) circle (2pt);
    
    % Subscript label
    \node[font=\sffamily] at (0, -1.8) {\textcolor{afmgray}{$u_5^*$}};
  \end{scope}

  % =========================================================
  % SIDE LEGEND (Right Panel)
  % =========================================================
  \begin{scope}[shift={(6.2, -1.2)}]
    % Outer Frame Box
    \draw[afmlinegray, thick, rounded corners=4pt, fill=gray!3] (0, -0.1) rectangle (4.2, 2.9);
    
    % Legend Header
    % \node[anchor=west, font=\sffamily\small] at (0.2, 3.1) {Legend \& Elements};
    % \draw[afmlinegray, thin] (0.2, 2.9) -- (4.0, 2.9);

    % 1. Blue Circle
    \draw[afmblue, ultra thick] (0.5, 2.4) circle (0.15);
    \node[anchor=west, font=\sffamily\scriptsize] at (0.85, 2.4) {Row-$\ell_2$ ball};

    % 2. Orange Box
    \draw[afmorange, ultra thick] (0.35, 1.75) rectangle (0.65, 2.05);
    \node[anchor=west, font=\sffamily\scriptsize] at (0.85, 1.9) {Max-entry ball};

    % 3. Green Fill
    \fill[afmgreen!70!white] (0.35, 1.25) rectangle (0.65, 1.55);
    \draw[afmorange, thick] (0.35, 1.25) rectangle (0.65, 1.55);
    \node[anchor=west, font=\sffamily\scriptsize] at (0.85, 1.4) {Shared intersection};

    % 4. Magenta Vector
    \draw[->, afmmagenta, line width=2pt] (0.35, 0.9) -- (0.65, 0.9);
    \fill[afmmagenta] (0.65, 0.9) circle (2pt);
    \node[anchor=west, font=\sffamily\scriptsize] at (0.85, 0.9) {AF-Muon update};

    % 5. Gray Setting
    \draw[afmgray, thick, dashed] (0.35, 0.25) rectangle (0.65, 0.55);
    \draw[->, afmgray, thick] (0.35, 0.4) -- (0.65, 0.4);
    \node[anchor=west, font=\sffamily\scriptsize] at (0.85, 0.4) {Comparison Setting};
  \end{scope}

\end{tikzpicture}
